Algorithmic Verification of Continuous and Hybrid Systems

We provide a tutorial introduction to reachability computation, a class of computational techniques that exports verification technology toward continuous and hybrid systems. For open under-determined systems, this technique can sometimes replace an infinite number of simulations.

==> eptcsdata.tex <==
\providecommand{\firstpage}{48}
\providecommand{\publicationstatus}{L. Clemente and L. Holik (Eds.): 15th International Workshop on\\
Verification of Infinite-State Systems (INFINITY'13)\\
EPTCS 140, 2014, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.140.4}{10.4204/EPTCS.140.4}}
\pdfoutput=1

